SQLucid: Grounding Natural Language Database Queries with Interactive Explanations

Though recent advances in machine learning have led to significant improvements in natural language interfaces for databases, the accuracy and reliability of these systems remain limited, especially in high-stakes domains. This paper introduces SQLucid, a novel user interface that bridges the gap between non-expert users and complex database querying processes. SQLucid addresses existing limitations by integrating visual correspondence, intermediate query results, and editable step-by-step SQL explanations in natural language to facilitate user understanding and engagement. This unique blend of features empowers users to understand and refine SQL queries easily and precisely. Two user studies and one quantitative experiment were conducted to validate SQLucid's effectiveness, showing significant improvement in task completion accuracy and user confidence compared to existing interfaces. Our code is available at https://github.com/magic-YuanTian/SQLucid.

==> table/accuracy_table.tex <==


% \usepackage{booktabs}


\begin{table}
\centering
\begin{tabular}{lcc} 
\toprule
      & \textbf{Task completion accuracy} & \textbf{SD} \\
        \midrule
no interaction     & 49.08\%  & 8\%     \\
MISP~\cite{misp}  & 57.01\%  & 29\%     \\
DIY~\cite{diy}   & 67.97\%   & 19\%   \\
STEPS & \textbf{85.81\%}   & 12\%   \\
\bottomrule
\end{tabular}
\caption{The Accuracy of Completed Tasks (i.e., \# of correctly completed tasks divided by \# of completed tasks).
\textcolor{blue}{Participants can correctly solve 49.08\% of tasks without using interactive tools.}
% User Performance (best results in bold). For all metrics, an ANOVA test indicated statistically significant mean differences across 3 tools ($p$-value < 0.01).
}
\label{tab:task_accuracy}
\end{table}

==> table/designs.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
\caption{Interactive designs for non-expert users}
\begin{tblr}{
  cell{2}{1} = {r=3}{},
  cell{5}{1} = {r=3}{},
  vline{2-3} = {2,3,4,5,6,7}{},
  vline{3} = {3-4,6-7}{},
  hline{1,8} = {-}{0.1em},
  hline{2,5} = {-}{},
  hline{3-4,6-7} = {2-3}{},
}
                                    & \textbf{Option}  & \textbf{Drawback}                                                     \\
\textbf{Understandable explanation} & Natural language & Hard to understand when the explanation is lengthy                    \\
                                    & Graph            & Hard to understand for complex SQL operations \\
                                    & Data transformation       & Hard to follow when the data schema is complex                                                                    \\
\textbf{Operatable feedback}        & Natural language & High-level instructions may lead to uncontrollable output             \\
                                    & Selection        & Not flexible                                                          \\
                                    & Graph edits      & Expertise required \& challenging for complex operations       
\end{tblr}
\label{tab:design}
\end{table}

==> table/expertise.tex <==
% \begin{table}
% \centering
% \resizebox{0.32\textwidth}{!}{%
% \begin{tabular}{lccc}
% \toprule
%   & \textbf{End-user}
%   & \textbf{Novice} 
%   & \textbf{Expert} \\ 
%   \midrule

% MISP~\cite{misp}        & 1.7   & 1.4    & 2.3      \\
% DIY~\cite{diy}     & 3.6   &  3.5    &  3.5     \\
% STEPS       & 5.6       & 5.7  & 6.0\\ 
% \bottomrule
% \end{tabular}%
% }
% \caption{ Tasks correctly completed by users with different
% levels of SQL expertise.}
% \label{tab:expertise}
% \end{table}



\begin{table}
\centering
\resizebox{0.55\linewidth}{!}{
\begin{tblr}{
  cells = {l},
  row{1} = {c},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  cell{1}{6} = {c=2}{},
  vline{2} = {1}{},
  vline{2,4,6} = {2-5}{},
  hline{1,6} = {-}{0.08em},
  hline{2} = {2-7}{},
  hline{3} = {-}{},
}
%      & \textbf{End-user} &      & \textbf{Novice}  &      & \textbf{Expert}  &      \\
%      & \textbf{\#Corr.}  & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   \\
%MISP~\cite{misp}  & 1.7      & 0.95 & 1.4     & 0.70 & 2.3     & 1.26 \\
%DIY~\cite{diy}   & 3.6      & 1.07 & 3.5     & 1.27 & 3.5     & 1.29 \\
%STEPS & 5.6      & 0.70 & 5.7     & 1.06 & 6.0     & 1.41 
%JKK Note: I transposed this so readers can easily look down a column and see that as expertise varies the numbers stay the same
      & \textbf{MISP~\cite{misp}} &      & \textbf{DIY~\cite{diy}}  &      & \textbf{STEPS}  &      \\
      & \textbf{\#Corr.}  & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   \\
End-User & 1.7 & 0.95 & 3.6 & 1.07 & 5.6 & 0.70 \\
Novice & 1.4 & 0.70   & 3.5 & 1.27   & 5.7 & 1.06   \\
Expert & 2.3 & 1.26   & 3.5 & 1.29   & 6.0 & 1.41
\end{tblr}
}
\caption{ Tasks correctly completed by users with different
levels of SQL expertise.}
\label{tab:expertise}
\end{table}

==> table/expertise_difficulty.tex <==
% \begin{table}[ht]
%     \centering
%         \begin{adjustbox}{valign=b}
%             \begin{minipage}{0.9\linewidth}
%                 \centering
%                 \resizebox{\linewidth}{!}{
%                     \begin{tblr}{
%                         cells = {l},
%                         row{1} = {c},
%                         cell{1}{2} = {c=2}{},
%                         cell{1}{4} = {c=2}{},
%                         cell{1}{6} = {c=2}{},
%                         vline{2} = {1}{},
%                         vline{2,4,6} = {2-5}{},
%                         hline{1,6} = {-}{0.08em},
%                         hline{2} = {2-7}{},
%                         hline{3} = {-}{},
%                     }
%                           & \textbf{MISP~\cite{misp}} &      & \textbf{DIY~\cite{diy}}  &      & \textbf{{\tool}}  &      \\
%                           & \textbf{\#Corr.}  & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   \\
%                     End-User & 1.6 & 0.91 & 3.3 & 1.13 & 5.4 & 0.91 \\
%                     Novice & 1.4 & 0.67   & 3.5 & 1.27   & 5.7 & 1.06   \\
%                     Expert & 2.2 & 1.10   & 3.8 & 1.30   & 5.9 & 1.22
%                     \end{tblr}
%                 }
%                 %\vspace{5pt}
%                 \caption{Tasks correctly completed by users with different levels of SQL expertise.}
%                 \label{tab:expertise}
%             \end{minipage}
%         \end{adjustbox}
%     \hfill
%         \begin{adjustbox}{valign=b}
%             \begin{minipage}{0.9\linewidth}
%                 \centering
%                 \resizebox{\linewidth}{!}{
%                     \begin{tblr}{
%                         cells = {l},
%                         row{1} = {c},
%                         cell{1}{2} = {c=2}{},
%                         cell{1}{4} = {c=2}{},
%                         cell{1}{6} = {c=2}{},
%                         vline{2} = {1}{},
%                         vline{2,4,6} = {2-6}{},
%                         hline{1,7} = {-}{0.08em},
%                         hline{2} = {2-7}{},
%                         hline{3} = {-}{},
%                     }
%                           & \textbf{MISP~\cite{misp}} &      & \textbf{DIY~\cite{diy}}  &      & \textbf{{\tool}}  &      \\
%                           & \textbf{\#Corr.}  & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   \\
%                     Easy    & 0.81 & 0.74     & 1.40 & 0.69  & 1.62 &  0.50 \\
%                     Medium  & 0.49 & 0.62   & 1.19 & 0.72   & 1.48 & 0.60   \\
%                     Hard    & 0.21 & 0.51   & 0.54 & 0.61   & 1.39 & 0.58  \\
%                     Extra hard  & 0.12 & 0.31   & 0.35 & 0.63   & 1.14 & 0.66  
%                     \end{tblr}
%                 } 
                
%                 \caption{Tasks correctly completed in different levels of task difficulty.}
%                 \label{tab:difficulty}
%                 \vspace{-10pt}
%             \end{minipage}
%         \end{adjustbox}
% \end{table}





\begin{table}[ht]
    \centering
    \begin{adjustbox}{valign=b}
        \begin{minipage}{0.9\linewidth}
            \centering
            \resizebox{\linewidth}{!}{
                \begin{tblr}{
                    cells = {l},
                    row{1} = {c},
                    cell{1}{2} = {c=2}{},
                    cell{1}{4} = {c=2}{},
                    cell{1}{6} = {c=2}{},
                    vline{2} = {1}{},
                    vline{2,4,6} = {2-5}{},
                    hline{1,6} = {-}{0.08em},
                    hline{2} = {2-7}{},
                    hline{3} = {-}{},
                    rowsep = 1pt, % Reduces space between rows
                }
                      & \textbf{MISP~\cite{misp}} &      & \textbf{DIY~\cite{diy}}  &      & \textbf{{\tool}}  &      \\
                      & \textbf{\#Corr.}  & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   \\
                End-User & 1.6 & 0.91 & 3.3 & 1.13 & 5.4 & 0.91 \\
                Novice & 1.4 & 0.67   & 3.5 & 1.27   & 5.7 & 1.06   \\
                Expert & 2.2 & 1.10   & 3.8 & 1.30   & 5.9 & 1.22
                \end{tblr}
            }
            \caption{Tasks correctly completed by users with different levels of SQL expertise.}
            \label{tab:expertise}
        \end{minipage}
    \end{adjustbox}
\end{table}

\begin{table}[ht]
    \centering
    \begin{adjustbox}{valign=b}
        \begin{minipage}{0.9\linewidth}
            \centering
            \resizebox{\linewidth}{!}{
                \begin{tblr}{
                    cells = {l},
                    row{1} = {c},
                    cell{1}{2} = {c=2}{},
                    cell{1}{4} = {c=2}{},
                    cell{1}{6} = {c=2}{},
                    vline{2} = {1}{},
                    vline{2,4,6} = {2-6}{},
                    hline{1,7} = {-}{0.08em},
                    hline{2} = {2-7}{},
                    hline{3} = {-}{},
                    rowsep = 1pt, % Reduces space between rows
                }
                      & \textbf{MISP~\cite{misp}} &      & \textbf{DIY~\cite{diy}}  &      & \textbf{{\tool}}  &      \\
                      & \textbf{\#Corr.}  & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   \\
                Easy    & 0.81 & 0.74     & 1.40 & 0.69  & 1.62 &  0.50 \\
                Medium  & 0.49 & 0.62   & 1.19 & 0.72   & 1.48 & 0.60   \\
                Hard    & 0.21 & 0.51   & 0.54 & 0.61   & 1.39 & 0.58  \\
                Extra hard  & 0.12 & 0.31   & 0.35 & 0.63   & 1.14 & 0.66  
                \end{tblr}
            } 
            \caption{Tasks correctly completed in different levels of task difficulty.}
            \label{tab:difficulty}
        \end{minipage}
    \end{adjustbox}
\end{table}


==> table/rule_table1.tex <==
\begin{table}[t]

\caption{Translation rules for SQL elements}
\label{tab:rule1}
\resizebox{0.8\linewidth}{!}{
    \centering
    \begin{tabular}{ll}
    \hline
    \textbf{SQL Elements} & \textbf{Translation}\\
    \hline
    % \hline
    \texttt{SELECT} & Return \\ 
    \texttt{FROM} & In table \\ 
    \texttt{JOIN} & and table \\ 
    \texttt{WHERE} & Keep the records where \\ 
    \texttt{GROUP BY} & Group the records based on \\ 
    \texttt{HAVING} & Keep the groups where \\ 
    \texttt{ORDER BY} & Sort the records based on \\ 
    % \texttt{ORDER BY COUNT(*)} & Sort groups based on the number \\ 
    % &  of records in each group\\
    \texttt{LIMIT 1} & return the first record \\
    \texttt{LIMIT num} & return the top \texttt{{num}} records \\
    \texttt{*} & all the records \\
    $\texttt{col}_1, \texttt{col}_2$ & the $\texttt{\{col}_1$\} and the $\texttt{\{col}_2$\} \\
    $\texttt{c}_1\, \texttt{c}_2\, \texttt{c}_3$ &  the $\texttt{\{c}_1$\}, the $\texttt{\{c}_2$\} and the $\texttt{\{c}_3$\}\\
    \texttt{T.col} & \texttt{\{col\}} of \texttt{\{T\}} \\ 
    \texttt{COUNT(col)} & the number of \texttt{\{col\}} \\ 
    \texttt{COUNT(*)} & the number of records \\ 
    \texttt{AVG(col)} & the average value of \texttt{\{col\}} \\ 
    \texttt{MAX(col)} & the maximum value of \texttt{\{col\}} \\ 
    \texttt{MIN(col)} & the minimum value of \texttt{\{col\}} \\ 
    \texttt{SUM(col)} & the sum value of \texttt{\{col\}} \\ 
    \texttt{ASC} & in ascending order \\ 
    \texttt{DESC} & in descending order \\ 
    \texttt{=} & is \\ 
    \texttt{!=} & is not \\ 
    \texttt{>} & is greater than \\ 
    \texttt{>=} & is greater than or equal to \\ 
    \texttt{<} & is less than \\ 
    \texttt{<=} & is less than or equal to \\ 
    \texttt{IN} & is in \\ 
    \texttt{NOT IN} & is not in \\ 
    \texttt{BETWEEN} & is between \\ 
    \texttt{LIKE} & is in the form of \\ 
    \texttt{NOT LIKE} & is not in the form of \\ 
    \hline
    \end{tabular}
}
\end{table}






% \begin{table}[t]
% \resizebox{0.8\linewidth}{!}{
%     \centering
%     \begin{tabular}{ll}
%     \hline
%     \textbf{SQL Elements} & \textbf{Translation}\\
%     \hline
%     % \hline
%     {\texttt{q$_1$ INTERSECT q$_2$} \\ \\ \\ \\} & 
%     {Start the first query: \\  
%     \textsc{Translate}(q$_1$); \\
%      Start the second query; \\ 
%      \textsc{Translate}(q$_2$); \\
%      Return the intersection of them;}


     
%     \texttt{NOT LIKE} & is not in the form of \\ 
%     \hline
%     \end{tabular}
% }
% \caption{Translation rules for SQL compound}
% \label{tab:rule2}
% \end{table}







==> table/rule_table2.tex <==
% \usepackage{tabularray}
% \begin{table}[!h]
% \centering
% \caption{Translation rules for SQL compound}
% \label{tab:rule2}
% \begin{tblr}{
%   row{1} = {l},
%   cell{2}{1} = {r=5}{},
%   cell{7}{1} = {r=5}{},
%   cell{12}{1} = {r=5}{},
%   cell{17}{1} = {r=5}{},
%   % hline{1-2,22} = {-}{},
%   hline{1-2,7,12,17,22} = {-}{},
% }
% \textbf{SQL compound}   & \textbf{Translation}                            \\
% q$_1$ \texttt{INTERSECT} q$_2$     & Start the first query:                          \\
%                         & \textsc{Translate} (q$_1$);                               \\
%                         & Start the second query;                         \\
%                         & \textsc{Translate} (q$_2$);                               \\
%                         & Return the intersection of them;                \\
% q$_1$ \texttt{UNION} $q_2$         & Start the first query q$_1:$                    \\
%                         & \textsc{Translate} (q$_1);$                               \\
%                         & Start the second query:                         \\
%                         & \textsc{Translate} (q$_2);$                               \\
%                         & Return the union of them.                       \\
% q$_1$ \texttt{EXCEPT} $q_2$        & Start the first query:                          \\
%                         & \textsc{Translate} (q$_1);$                               \\
%                         & Start the second query:                         \\
%                         & \textsc{Translate} (q$_2);$                               \\
%                         & Return the records in q$_1 but not in q_2.$     \\
% ... col \texttt{IN/NOT IN} q$_1$ & Start the first query:                          \\
%                         & \textsc{Translate} (q$_1);$                               \\
%                         & Start the second query:                         \\
%                         & \textsc{Translate} (...);                                 \\
%                         & Keep the records where \{col\} in/not in q$_1.$ 
% \end{tblr}
% \end{table}

\begin{table}[t]

\caption{Translation rules for SQL compound}
\label{tab:rule2}
\resizebox{0.48\textwidth}{!}{
\centering

\begin{tabular}{ll}
\hline
\textbf{SQL compound} & \textbf{Translation}\\
\hline
% \hline
\specialrule{0em}{2pt}{2pt}
\multirow{}{}{\texttt{q$_1$ INTERSECT q$_2$}}  & Start the first query: \\ & \textsc{Translate}(q$_1$); \\
                                & Start the second query; \\ & \textsc{Translate}(q$_2$); \\
                                & Return the intersection of them; \\
\specialrule{0.002em}{2pt}{3.5pt}

\multirow{}{}{\texttt{q$_1$ UNION q$_2$}}  & Start the first query {q$_1$}: \\ & \textsc{Translate}(q$_1$); \\
                                & Start the second query: \\ & \textsc{Translate}(q$_2$); \\
                                & Return the union of them. \\
\specialrule{0.002em}{2pt}{3.5pt}


\multirow{}{}{\texttt{q$_1$ EXCEPT q$_2$}}   & Start the first query: \\ & \textsc{Translate}(q$_1$); \\
                                & Start the second query: \\
                                & \textsc{Translate}(q$_2$); \\
                                & Return the records in {q$_1$} but not in {q$_2$}. \\

\specialrule{0.002em}{2pt}{3.5pt}


\multirow{}{}{... \texttt{col IN/NOT IN q$_1$}}   & Start the first query: \\
& \textsc{Translate}(q$_1$); \\
                                & Start the second query: \\
                                & \textsc{Translate}(...); \\
                                & Keep the records where \{col\} in/not in {q$_1$}. \\


                                
\specialrule{0em}{2pt}{2pt}
\hline
\end{tabular}
}
\end{table}

==> table/rule_table3.tex <==




\begin{table}
\resizebox{0.32\textwidth}{!}{
\centering

\begin{tabular}{ll}
\hline
\textbf{SQL compound} & \textbf{Translation}\\
\hline
% \hline
\specialrule{0em}{2pt}{2pt}
\multirow{5}{*}{\texttt{q$_1$ INTERSECT q$_2$}}  & Start the first query: \\ & \textsc{Translate}(q$_1$); \\
                                & Start the second query; \\ & \textsc{Translate}(q$_2$); \\
                                & Return the intersection of them; \\
\specialrule{0.002em}{2pt}{3.5pt}

\multirow{}{}{\texttt{q$_1$ UNION q$_2$}}  & Start the first query {q$_1$}: \\ & \textsc{Translate}(q$_1$); \\
                                & Start the second query: \\ & \textsc{Translate}(q$_2$); \\
                                & Return the union of them. \\
\specialrule{0.002em}{2pt}{3.5pt}


\multirow{}{}{\texttt{q$_1$ EXCEPT q$_2$}}   & Start the first query: \\ & \textsc{Translate}(q$_1$); \\
                                & Start the second query: \\
                                & \textsc{Translate}(q$_2$); \\
                                & Return the records in {q$_1$} but not in {q$_2$}. \\

\specialrule{0.002em}{2pt}{3.5pt}


\multirow{}{}{... \texttt{col IN/NOT IN q$_1$}}   & Start the first query: \\
& \textsc{Translate}(q$_1$); \\
                                & Start the second query: \\
                                & \textsc{Translate}(...); \\
                                & Keep the records where \{col\} in/not in {q$_1$}. \\


                                
\specialrule{0em}{2pt}{2pt}
\hline
\end{tabular}
}
\caption{NL explanation translation rules for SQL compound}
\label{tab:explanation2}
\end{table}


==> table/task_completion_accuracy_figure_table.tex <==
% \begin{figure}[ht]
%     \centering

%     % Set the space above the caption
%     \setlength{\abovecaptionskip}{10pt}
    
%     % First minipage for the table
%     \begin{adjustbox}{valign=b}
%         \begin{minipage}[h]{0.52\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{figures/performance4.png}
%             \captionof{figure}{Distribution of completed tasks categories (correct, incorrect, skipped, remained) with different tools.}
%             \label{fig:performance}
%         \end{minipage}
%     \end{adjustbox}
%     \hfill
%     % Second minipage for the figure
%     \begin{adjustbox}{valign=b}
%         \begin{minipage}[h]{0.45\linewidth}
%             \centering
            
%             \begin{tabular}{lcc} 
%                 \toprule
%                       & \textbf{Task completion accuracy} & \textbf{SD} \\
%                 \midrule
%                 %no interaction     & 49.08\%  & 8\%     \\
%                 MISP~\cite{misp}  & 57\%  & 29\%     \\
%                 DIY~\cite{diy}   & 68\%   & 19\%   \\
%                 STEPS & \textbf{86\%}   & 12\%   \\
%                 \bottomrule
%             \end{tabular}
%             \vspace{10pt} % Adjust this value to match the space above the figure's caption
%             \captionof{table}{The Accuracy of Completed Tasks (i.e., \# of correctly completed tasks divided by \# of completed tasks).} % <-- here's the fix
%             %\textcolor{blue}{Participants can correctly solve 49.08\% of tasks without using interactive tools.}}
%             \label{tab:task_accuracy}
%         \end{minipage}
%     \end{adjustbox}
% \end{figure}



\begin{figure}[ht]
    \centering
    \setlength{\abovecaptionskip}{10pt}
    % First minipage for the figure
    \begin{minipage}{\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{figures/performance5.png}
        \captionof{figure}{Distribution of completed tasks categories (correct, incorrect, skipped, remained) with different tools.}
        \label{fig:performance}
    \end{minipage}
    \hfill
    % Second minipage for the table
    \raisebox{-0.495cm}{%  Adjust -1cm to your desired value
    \begin{minipage}{\linewidth}
        \centering
        \begin{tabular}{lcc}
            \toprule
                  & \textbf{Task completion accuracy} & \textbf{SD} \\
            \midrule
            MISP~\cite{misp}  & 56\%  & 30\% \\
            DIY~\cite{diy}   & 67\%   & 20\% \\
            {\tool} & \textbf{85\%}   & 13\% \\
            \bottomrule
        \end{tabular}
        \vspace{10pt}
        \captionof{table}{The Accuracy of Completed Tasks (i.e., \# of correctly completed tasks divided by \# of completed tasks).}
        \label{tab:task_accuracy}
    \end{minipage}
    }

\end{figure}



% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/performance5.png}
%     \vspace{-1mm}
%     \caption{Distribution of completed tasks categories (correct, incorrect, skipped, remained) with different tools.}
%     \label{fig:performance}
% \end{figure}


% \begin{table}[ht]
%     \centering
%     \begin{tabular}{lcc}
%         \toprule
%               & \textbf{Task completion accuracy} & \textbf{SD} \\
%         \midrule
%         MISP~\cite{misp}  & 56\%  & 30\% \\
%         DIY~\cite{diy}   & 67\%   & 20\% \\
%         {\tool} & \textbf{85\%}   & 13\% \\
%         \bottomrule
%     \end{tabular}
%     \vspace{2mm}
%     \caption{The Accuracy of Completed Tasks (i.e., \# of correctly completed tasks divided by \# of completed tasks).}
%     \label{tab:task_accuracy}
% \end{table}

    



==> table/task_difficulty_correct.tex <==



\begin{table}
\centering
\resizebox{0.55\linewidth}{!}{
\begin{tblr}{
  cells = {l},
  row{1} = {c},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=2}{},
  cell{1}{6} = {c=2}{},
  vline{2} = {1}{},
  vline{2,4,6} = {2-6}{},
  hline{1,7} = {-}{0.08em},
  hline{2} = {2-7}{},
  hline{3} = {-}{},
}

      & \textbf{MISP~\cite{misp}} &      & \textbf{DIY~\cite{diy}}  &      & \textbf{STEPS}  &      \\
      & \textbf{\#Corr.}  & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   & \textbf{\#Corr.} & \textbf{SD}   \\
Easy    & 0.83 & 0.70     & 1.38 & 0.65  & 1.63 &  0.49 \\
Medium  & 0.5 & 0.66   & 1.21 & 0.72   & 1.50 & 0.59   \\
Hard    & 0.21 & 0.51   & 0.58 & 0.65   & 1.46 & 0.59  \\
Extra hard  & 0.13 & 0.34   & 0.38 & 0.65   & 1.13 & 0.68  
\end{tblr}
}
\caption{Tasks correctly completed in different levels of difficulty.}
\label{tab:difficulty}
\end{table}

==> table/tasks.tex <==
% % \usepackage{tabularray}
% \begin{table*}
% \centering
% \begin{tblr}{
%   cells = {l},
%   cell{2}{1} = {r=6}{},
%   cell{8}{1} = {r=6}{},
%   cell{14}{1} = {r=6}{},
%   cell{20}{1} = {r=6}{},
%   vline{2} = {2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24, 25}{},
%   hline{1,26} = {-}{0.08em},    
%   hline{2,8,14,20} = {-}{},
%   hline{3-7,9-13,15-19,21-25} = {2-3}{},
% }
%               & \textbf{Task} & \textbf{Database} \\
% \textbf{Easy}          
%               & {List the name of teachers whose hometown is not \\  “Little Lever Urban District}    & course\_teach        \\
%               & How many countries speak both English and Dutch?    & world\_1        \\
%               & List all the student details in reversed lexicographical order.    & 1        \\
%               & What are the names of the singers who are not French citizens?    & singer        \\
%               & How many ships ended up being 'Captured'?    & battle\_death        \\
%               & {In which years cars were produced weighing no less than 3000 \\ and no more than 4000?}    & car\_1        \\
% \textbf{Medium}        
%               & Which airlines have less than 200 flights?    & flights\_2        \\
%               & {Who is the earliest graduate of the school? \\ List the first name, middle name, and last name.}    & student\_transcripts\_tracking        \\
%               & {What are the countries having at least one car maker? List name and id.}    & car\_1        \\
%               & {What is the official language used in the country the \\ name of whose head of state is Beatrix?}    & world\_1        \\
%               & Find all airlines that have at least 10 flights.    & flights\_2        \\
%               & {What are the codes of countries where Spanish is spoken by \\ the largest percentage of people?}    & world\_1        \\
% \textbf{Hard}          
%               & {What are the ids and names of the battles that led to more than 10 \\ people killed in total?}    & battle\_death        \\
%               & {What is the maximum number of times that a course \\ shows up in different transcripts and \\ what is that course's enrollment id?}    & student\_transcripts\_tracking        \\
%               & {What are the first names of the students who live in \\ Haiti permanently or have the cell phone number 09700166582?}    & student\_transcripts\_tracking        \\
%               & How many car models are produced in the USA?    & car\_1        \\
%               & Show the name of the teacher for the math course.    & course\_teach        \\
%               & Return the names of friends of the high school student Kyle.    & network\_1        \\
% \textbf{Extra\\hard} 
%               & {What is the first name of every student who has a dog \\ but does not have a cat?}    & pets\_1        \\
%               & {Who owns the youngest dog? Give me his or her last name.}    & dog\_kennels        \\
%               & {What is the series name and country \\ of all TV channels that  are playing cartoons \\ directed by Ben Jones and cartoons directed by Michael Chang?}    & tvshow        \\
%               & {Which owner has paid the largest amount of \\ money in total for their dogs?  Show the owner id and zip code.}    & dog\_kennels        \\
%               & {What is the area code in which the most voters voted?}    & voter\_1        \\
%               & {What is the maximum horsepower and the make of the \\ car models with 3 cylinders?}    & car\_1        
% \end{tblr}
% \caption{User study tasks}
% \label{tab:tasks}
% \end{table*}














% \usepackage{tabularray}
\begin{table*}
\centering
\captionsetup{labelformat=empty}
\begin{tblr}{
  cells = {l},
  column{1} = {c},
  % row{1} = {c},
  % column{3} = {r},
  cell{2}{1} = {r=6}{},
  cell{8}{1} = {r=6}{},
  cell{14}{1} = {r=6}{},
  cell{20}{1} = {r=6}{},
  vline{2} = {2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20,21,22,23,24, 25}{},
  hline{1,26} = {-}{0.08em},    
  hline{2,8,14,20} = {-}{},
  hline{3-7,9-13,15-19,21-25} = {2-3}{},
}
                                & \textbf{Task}                                                                                                                                         & \textbf{Database}              \\
\textbf{Easy}                   & {List the name of teachers whose hometown is not \\  “Little Lever Urban District}                                                                    & course\_teach                  \\
                                & What is the abbreviation for airline "JetBlue Airways"?                                                                                                      & flight\_2                       \\
                                & List all the student details in reversed lexicographical order.                                                                                       & student\_transcripts\_tracking \\
                                & What are the names of the singers who are not French citizens?                                                                                        & singer                         \\
                                & How many ships ended up being 'Captured'?                                                                                                             & battle\_death                  \\
                                & {In which years cars were produced weighing \\no less than 3000 and no more than 4000?}                                                               & car\_1                         \\
\textbf{Medium}                 & Which airlines have less than 200 flights?                                                                                                            & flights\_2                     \\
                                & {Who is the earliest graduate of the school? \\ List the first name, middle name, and last name.}                                                     & student\_transcripts\_tracking \\
                                & {What are the countries having at least one car maker? \\ List name and id.}                                                                          & car\_1                         \\
                                & {What is the official language used in the country the \\ name of whose head of state is Beatrix?}                                                    & world\_1                       \\
                                & Find all airlines that have at least 10 flights.                                                                                                      & flights\_2                     \\
                                & {What are the codes of countries where Spanish is spoken by \\ the largest percentage of people?}                                                     & world\_1                       \\
\textbf{Hard}                   & {What are the ids and names of the battles that led to\\more than 10 people killed in total?}                                                         & battle\_death                  \\
                                & {What is the maximum number of times that a course \\ shows up in different transcripts and \\ what is that course's enrollment id?}                  & student\_transcripts           \\
                                & {What are the first names of the students who live in Haiti \\permanently or have the cell phone number 09700166582?}                                 & student\_transcripts\_tracking \\
                                & How many car models are produced in the USA?                                                                                                          & car\_1                         \\
                                & Show the name of the teacher for the math course.                                                                                                     & course\_teach                  \\
                                & Return the names of friends of the high school student Kyle.                                                                                          & network\_1                     \\
{\textbf{Extra}\\\textbf{hard}} & {What is the first name of every student who has a dog \\ but does not have a cat?}                                                                   & pets\_1                        \\
                                & Who owns the youngest dog? Give me his or her last name.                                                                                              & dog\_kennels                   \\
                                & {What is the series name and country of all TV channels \\that  are playing cartoons directed by Ben Jones and \\cartoons directed by Michael Chang?} & tvshow                         \\
                                & {Which owner has paid the largest amount of money in \\total for their dogs?  Show the owner id and zip code.}                                        & dog\_kennels                   \\
                                & What is the area code in which the most voters voted?                                                                                                 & voter\_1                       \\
                                & {What is the maximum horsepower and the make of the \\ car models with 3 cylinders?}                                                                  & car\_1                         
\end{tblr}
\caption{User study tasks}
\label{tab:tasks}
\end{table*}

==> table/tasks2.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
\captionsetup{labelformat=empty}
\caption{User study tasks}
\label{tab:tasks}
\begin{tblr}{
  column{1} = {c},
  cell{2}{1} = {r=6}{},
  cell{8}{1} = {r=6}{},
  cell{14}{1} = {r=6}{},
  cell{20}{1} = {r=6}{},
  vline{2} = {2,8,14,20}{},
  hline{1-2,8,14,20,26} = {-}{},
  hline{3-7,9-13,15-19,21-25} = {2-3}{},
}
                                & \textbf{Task}                                                                                                                                             & \textbf{Ground truth SQL query}                                                                                                                                                                                                                                                                                                          \\
\textbf{Easy}                   & {List the name of teachers whose hometown \\is not “Little Lever Urban District}                                                                          & {SELECT name FROM teacher \\WHERE hometown != "little lever urban district”}                                                                                                                                                                                                                                                             \\
                                & {What is the abbreviation \\for airline "JetBlue Airways" ?}                                                                                              & {SELECT Abbreviation FROM AIRLINES \\WHERE Airline = "JetBlue Airways”}                                                                                                                                                                                                                                                                  \\
                                & {List all the student details \\in reversed lexicographical order.}                                                                                       & {SELECT other\_student\_details FROM Students \\ORDER BY other\_student\_details DESC}                                                                                                                                                                                                                                                   \\
                                & {What are the names of the \\singers who are not French citizens?}                                                                                        & {SELECT Name FROM singer \\WHERE Citizenship != "France”}                                                                                                                                                                                                                                                                                \\
                                & How many ships ended up being 'Captured'?                                                                                                                 & {SELECT COUNT(*) FROM ship \\WHERE disposition\_of\_ship = 'Captured’}                                                                                                                                                                                                                                                                   \\
                                & {In which years cars were produced weighing \\no less than 3000 and no more than 4000?}                                                                   & {SELECT DISTINCT year FROM cars\_data \\WHERE weight BETWEEN 3000 AND 4000}                                                                                                                                                                                                                                                              \\
\textbf{Medium}                 & Which airlines have less than 200 flights?                                                                                                                & {SELECT T1.Airline FROM AIRLINES AS T1 \\JOIN FLIGHTS AS T2 ON T1.uid = T2.Airline \\GROUP BY T1.Airline HAVING COUNT(*)  200}                                                                                                                                                                                                           \\
                                & {Who is the earliest graduate of the school? \\ List the first name, middle name, and last name.}                                                         & {SELECT first\_name , middle\_name , last\_name \\FROM Students ORDER BY date\_left ASC LIMIT 1}                                                                                                                                                                                                                                         \\
                                & {What are the countries having \\at least one car maker? \\ List name and id.}                                                                            & {SELECT T1.CountryName , T1.CountryId \\FROM COUNTRIES \\AS T1 JOIN CAR\_MAKERS AS T2 \\ON T1.CountryId = T2.Country \\GROUP BY T1.CountryId HAVING COUNT(*) = 1}                                                                                                                                                                        \\
                                & {What is the official language used \\in the country the name of \\whose head of state is Beatrix?}                                                       & {SELECT T2.Language FROM country AS T1 \\JOIN countrylanguage AS T2 \\ON T1.Code = T2.CountryCode \\WHERE T1.HeadOfState = "Beatrix" \\AND T2.IsOfficial = "T”}                                                                                                                                                                          \\
                                & Find all airlines that have at least 10 flights.                                                                                                          & {SELECT T1.Airline FROM AIRLINES \\AS T1 JOIN FLIGHTS AS T2 ON T1.uid = T2.Airline \\GROUP BY T1.Airline HAVING COUNT(*)  10}                                                                                                                                                                                                            \\
                                & {What are the codes of countries \\where Spanish is spoken by \\ the largest percentage of people?}                                                       & {SELECT CountryCode , MAX(Percentage) \\FROM countrylanguage \\WHERE language= "Spanish" GROUP BY CountryCode}                                                                                                                                                                                                                           \\
\textbf{Hard}                   & {What are the ids and names \\of the battles that led to\\more than 10 people \\killed in total?}                                                         & {SELECT T1.id , T1.name FROM battle AS T1 \\JOIN ship AS T2 ON T1.id = T2.lost\_in\_battle \\JOIN death AS T3 ON T2.id = T3.caused\_by\_ship\_id \\GROUP BY T1.id HAVING SUM(T3.killed)  10}                                                                                                                                             \\
                                & {What is the maximum number of times that \\a course shows up in different transcripts \\and what is that course's enrollment id?}                        & {SELECT COUNT(*) , student\_course\_id \\FROM Transcript\_Contents \\GROUP BY student\_course\_id \\ORDER BY COUNT(*) DESC LIMIT 1}                                                                                                                                                                                                      \\
                                & {What are the first names of the students who \\live in Haiti permanently or have the cell \\phone number 09700166582?}                                   & {SELECT T1.first\_name FROM students AS T1 \\JOIN addresses AS t2 \\ON T1.permanent\_address\_id = T2.address\_id \\WHERE T2.country = 'haiti' \\OR T1.cell\_mobile\_number = '09700166582’}                                                                                                                                             \\
                                & How many car models are produced in the USA?                                                                                                              & {SELECT COUNT(*) FROM MODEL\_LIST AS T1 \\JOIN CAR\_MAKERS AS T2 ON T1.Maker = T2.Id \\JOIN COUNTRIES AS T3\\ON T2.Country = T3.CountryId \\WHERE T3.CountryName = 'usa'}                                                                                                                                                                \\
                                & Show the name of the teacher for the math course.                                                                                                         & {SELECT T3.Name FROM course\_arrange AS T1 \\JOIN course AS T2 \\ON T1.Course\_ID = T2.Course\_ID \\JOIN teacher AS T3 \\ON T1.Teacher\_ID = T3.Teacher\_ID \\WHERE T2.Course = "Math"}                                                                                                                                                  \\
                                & {Return the names of \\friends of the high \\school student Kyle.}                                                                                        & {SELECT T3.name FROM Friend AS T1 JOIN Highschooler AS T2 \\ON T1.student\_id = T2.id JOIN Highschooler AS T3 \\ON T1.friend\_id = T3.id WHERE T2.name = "Kyle"}                                                                                                                                                                         \\
{\textbf{Extra}\\\textbf{hard}} & {What is the first name \\of every student \\who has a dog \\but does not \\have a cat?}                                                                  & {SELECT T1.fname , T1.age FROM student AS T1 JOIN has\_pet AS T2 \\ON T1.stuid = T2.stuid JOIN pets AS T3 ON T3.petid = T2.petid \\WHERE T3.pettype = 'dog' AND \\T1.stuid NOT IN \\(SELECT T1.stuid FROM student AS T1 JOIN has\_pet AS T2 \\ON T1.stuid = T2.stuid JOIN pets AS T3 ON T3.petid = T2.petid \\WHERE T3.pettype = 'cat')} \\
                                & {Who owns the youngest dog? \\Give me his or her last name.}                                                                                              & {SELECT T1.last\_name FROM Owners AS T1 JOIN Dogs AS T2 \\ON T1.owner\_id = T2.owner\_id WHERE T2.age = \\( SELECT MAX(age) FROM Dogs )}                                                                                                                                                                                                 \\
                                & {What is the series name and \\country of all TV channels \\that  are playing cartoons directed \\by Ben Jones and cartoons \\directed by Michael Chang?} & {SELECT T1.series\_name , T1.country FROM TV\_Channel AS T1 \\JOIN cartoon AS T2 ON T1.id = T2.Channel \\WHERE T2.directed\_by = 'Michael Chang' \\INTERSECT SELECT T1.series\_name , T1.country \\FROM TV\_Channel AS T1 JOIN cartoon AS T2 ON T1.id = T2.Channel \\WHERE T2.directed\_by = 'Ben Jones'}                                \\
                                & {Which owner has paid the largest \\amount of money in total for their dogs? \\~Show the owner id and zip code.}                                          & {SELECT T1.owner\_id , T1.zip\_code FROM Owners AS T1 JOIN Dogs \\AS T2 ON T1.owner\_id = T2.owner\_id JOIN Treatments AS T3 \\ON T2.dog\_id = T3.dog\_id \\GROUP BY T1.owner\_id \\ORDER BY sum(T3.cost\_of\_treatment) DESC LIMIT 1}                                                                                                   \\
                                & {What is the area code\\~in which the most voters voted?}                                                                                                 & {SELECT T1.area\_code FROM area\_code\_state AS T1 \\JOIN votes AS T2 ON T1.state = T2.state \\GROUP BY T1.area\_code \\ORDER BY COUNT(*) DESC LIMIT 1}                                                                                                                                                                                  \\
                                & {What is the maximum horsepower \\and the make of the car models \\with 3 cylinders?}                                                                     & {SELECT T2.horsepower , T1.Make FROM CAR\_NAMES AS T1 \\JOIN CARS\_DATA AS T2 ON T1.MakeId = T2.Id WHERE T2.cylinders = 3 \\ORDER BY T2.horsepower DESC LIMIT 1}                                                                                                                                                                         
\end{tblr}
\end{table}

==> table/tasks3.tex <==
% \usepackage{tabularray}
\begin{table*}
\centering
%\captionsetup{labelformat=empty}
\caption{User study tasks with ground truth SQLs (Easy \& Medium)}
\label{tab:tasks1}
\resizebox{0.85\textwidth}{!}{
\begin{tblr}{
  column{1} = {c},
  cell{2}{1} = {r=6}{},
  cell{8}{1} = {r=6}{},
  vline{2} = {2,3,4,5,6,7,8,9,10,11,12,13,14,15,16}{},
  hline{1-2} = {-}{},
  hline{8} = {-}{},
  hline{14} = {-}{},
  hline{3-14} = {2-3}{},
}
                & \textbf{Task Database}                                                                                                   & \textbf{Ground truth SQL query}                                                                                                                                   \\
\textbf{Easy}   & {List the name of teachers whose hometown \\is not “Little Lever Urban District. \\\textbf{(course\_teach)}}             & {SELECT name FROM teacher \\WHERE hometown != ``little lever urban district''}                                                                                      \\
                & {What is the abbreviation \\for airline ``JetBlue Airways'' ? \\\textbf{(flight\_2)}}                                      & {SELECT Abbreviation FROM AIRLINES \\WHERE Airline = ``JetBlue Airways''}                                                                                           \\
                & {List all the student details in \\reversed lexicographical order. \\\textbf{(student\_transcripts\_tracking)}}          & {SELECT other\_student\_details FROM Students \\ORDER BY other\_student\_details DESC}                                                                            \\
                & {What are the names of the \\singers who are not French citizens? \\\textbf{(singer)}}                                   & {SELECT Name FROM singer \\WHERE Citizenship != ``France''}                                                                                                         \\
                & {How many ships ended up being 'Captured'?\\\textbf{(battle\_death)}}                                                    & {SELECT COUNT(*) FROM ship \\WHERE disposition\_of\_ship = 'Captured’}                                                                                            \\
                & {In which years cars were produced weighing \\no less than 3000 and no more than 4000?\\\textbf{(car\_1)}}               & {SELECT DISTINCT year FROM cars\_data \\WHERE weight BETWEEN 3000 AND 4000}                                                                                       \\
\textbf{Medium} & {Which airlines have less than 200 flights?\\\textbf{(flights\_2)}}                                                      & {SELECT T1.Airline FROM AIRLINES AS T1 \\JOIN FLIGHTS AS T2 ON T1.uid = T2.Airline \\GROUP BY T1.Airline HAVING COUNT(*)  200}                                    \\
                & {Who is the earliest graduate of the school? \\ List the first name, middle name, and last name.\\\textbf{(flights\_2)}} & {SELECT first\_name , middle\_name , last\_name \\FROM Students ORDER BY date\_left ASC LIMIT 1}                                                                  \\
                & {What are the countries having \\at least one car maker? \\ List name and id.\\\textbf{(car\_1)}}                        & {SELECT T1.CountryName , T1.CountryId \\FROM COUNTRIES \\AS T1 JOIN CAR\_MAKERS AS T2 \\ON T1.CountryId = T2.Country \\GROUP BY T1.CountryId HAVING COUNT(*) = 1} \\
                & {What is the official language used \\in the country the name of \\whose head of state is Beatrix?\\\textbf{(world\_1)}} & {SELECT T2.Language FROM country AS T1 \\JOIN countrylanguage AS T2 \\ON T1.Code = T2.CountryCode \\WHERE T1.HeadOfState = ``Beatrix'' \\AND T2.IsOfficial = ``T''}   \\
                & {Find all airlines that have at least 10 flights.\\\textbf{(flights\_2)}}                                                & {SELECT T1.Airline FROM AIRLINES \\AS T1 JOIN FLIGHTS AS T2 ON T1.uid = T2.Airline \\GROUP BY T1.Airline HAVING COUNT(*)  10}                                     \\
                & {What are the codes of countries \\where Spanish is spoken by \\ the largest percentage of people?\\\textbf{(world\_1)}} & {SELECT CountryCode , MAX(Percentage) \\FROM countrylanguage \\WHERE language= ``Spanish'' GROUP BY CountryCode}                                                    
\end{tblr}
}
\end{table*}

==> table/tasks4.tex <==
% \usepackage{tabularray}
\begin{table*}
\centering
%\captionsetup{labelformat=empty}
\caption{User study tasks (Hard \& Extra Hard)}
\label{tab:tasks2}
\resizebox{0.9\textwidth}{!}{
\begin{tblr}{
  column{1} = {c},
  cell{2}{1} = {r=6}{},
  cell{8}{1} = {r=6}{},
  vline{2} = {2,3,4,5,6,7,8,9,10,11,12,13,14,15,16}{},
  hline{1-2} = {-}{},
  hline{8} = {-}{},
  hline{14} = {-}{},
  hline{3-14} = {2-3}{},
}
                                & \textbf{Task}                                                                                                                                                                 & \textbf{Ground truth SQL query}                                                                                                                                                                                                                                                                                                          \\
\textbf{Hard}                   & {What are the ids and names of the \\battles that led to more than 10 \\people killed in total?\\\textbf{(battle\_death)}}                                                    & {SELECT T1.id , T1.name FROM battle AS T1 \\JOIN ship AS T2 ON T1.id = T2.lost\_in\_battle \\JOIN death AS T3 ON T2.id = T3.caused\_by\_ship\_id \\GROUP BY T1.id HAVING SUM(T3.killed)  10}                                                                                                                                             \\
                                & {What is the maximum number of times that \\a course shows up in different transcripts \\and what is that course's enrollment id?\\\textbf{(student\_transcripts\_tracking)}} & {SELECT COUNT(*) , student\_course\_id \\FROM Transcript\_Contents \\GROUP BY student\_course\_id \\ORDER BY COUNT(*) DESC LIMIT 1}                                                                                                                                                                                                      \\
                                & {What are the first names of the students who \\live in Haiti permanently or have the cell \\phone number 09700166582?\\\textbf{(student\_transcripts\_tracking)}}            & {SELECT T1.first\_name FROM students AS T1 \\JOIN addresses AS t2 \\ON T1.permanent\_address\_id = T2.address\_id \\WHERE T2.country = 'haiti' \\OR T1.cell\_mobile\_number = '09700166582’}                                                                                                                                             \\
                                & {How many car models are produced in the USA?\\\textbf{(car\_1)}}                                                                                                             & {SELECT COUNT(*) FROM MODEL\_LIST AS T1 \\JOIN CAR\_MAKERS AS T2 ON T1.Maker = T2.Id \\JOIN COUNTRIES AS T3\\ON T2.Country = T3.CountryId \\WHERE T3.CountryName = 'usa'}                                                                                                                                                                \\
                                & {Show the name of the teacher for the math course.\\\textbf{(course\_teach)}}                                                                                                 & {SELECT T3.Name FROM course\_arrange AS T1 \\JOIN course AS T2 \\ON T1.Course\_ID = T2.Course\_ID \\JOIN teacher AS T3 \\ON T1.Teacher\_ID = T3.Teacher\_ID \\WHERE T2.Course = "Math"}                                                                                                                                                  \\
                                & {Return the names of friends of the high \\school student Kyle.\\\textbf{(network\_1)}}                                                                                       & {SELECT T3.name FROM Friend AS T1 JOIN Highschooler AS T2 \\ON T1.student\_id = T2.id JOIN Highschooler AS T3 \\ON T1.friend\_id = T3.id WHERE T2.name = "Kyle"}                                                                                                                                                                         \\
{\textbf{Extra}\\\textbf{hard}} & {What is the first name of every student \\who has a dog but does not have a cat?\\\textbf{(pets\_1)}}                                                                        & {SELECT T1.fname , T1.age FROM student AS T1 JOIN has\_pet AS T2 \\ON T1.stuid = T2.stuid JOIN pets AS T3 ON T3.petid = T2.petid \\WHERE T3.pettype = 'dog' AND \\T1.stuid NOT IN \\(SELECT T1.stuid FROM student AS T1 JOIN has\_pet AS T2 \\ON T1.stuid = T2.stuid JOIN pets AS T3 ON T3.petid = T2.petid \\WHERE T3.pettype = 'cat')} \\
                                & {Who owns the youngest dog? \\Give me his or her last name.\\\textbf{(dog\_kennels)}}                                                                                         & {SELECT T1.last\_name FROM Owners AS T1 JOIN Dogs AS T2 \\ON T1.owner\_id = T2.owner\_id WHERE T2.age = \\( SELECT MAX(age) FROM Dogs )}                                                                                                                                                                                                 \\
                                & {What is the series name and \\country of all TV channels \\that  are playing cartoons directed \\by Ben Jones and cartoons \\directed by Michael Chang?\\\textbf{(tvshow)}}  & {SELECT T1.series\_name , T1.country FROM TV\_Channel AS T1 \\JOIN cartoon AS T2 ON T1.id = T2.Channel \\WHERE T2.directed\_by = 'Michael Chang' \\INTERSECT SELECT T1.series\_name , T1.country \\FROM TV\_Channel AS T1 JOIN cartoon AS T2 ON T1.id = T2.Channel \\WHERE T2.directed\_by = 'Ben Jones'}                                \\
                                & {Which owner has paid the largest \\amount of money in total for their dogs? \\Show the owner id and zip code.\\\textbf{(dog\_kennels)}}                                      & {SELECT T1.owner\_id , T1.zip\_code FROM Owners AS T1 JOIN Dogs \\AS T2 ON T1.owner\_id = T2.owner\_id JOIN Treatments AS T3 \\ON T2.dog\_id = T3.dog\_id \\GROUP BY T1.owner\_id \\ORDER BY sum(T3.cost\_of\_treatment) DESC LIMIT 1}                                                                                                   \\
                                & {What is the area code in which the most \\voters voted?\\\textbf{(voter\_1)}}                                                                                                & {SELECT T1.area\_code FROM area\_code\_state AS T1 \\JOIN votes AS T2 ON T1.state = T2.state \\GROUP BY T1.area\_code \\ORDER BY COUNT(*) DESC LIMIT 1}                                                                                                                                                                                  \\
                                & {What is the maximum horsepower and the \\make of the car models with 3 cylinders?\\\textbf{(car\_1)}}                                                                        & {SELECT T2.horsepower , T1.Make FROM CAR\_NAMES AS T1 \\JOIN CARS\_DATA AS T2 ON T1.MakeId = T2.Id WHERE T2.cylinders = 3 \\ORDER BY T2.horsepower DESC LIMIT 1}                                                                                                                                                                         
\end{tblr}
}
\end{table*}

==> table/testtable.tex <==
% \usepackage{tabularray}
\begin{table}
\centering
% \captionsetup{labelformat=empty}
\caption{TEST}
\label{tab:tasks1}
\begin{tblr}{
  column{1} = {c},
  cell{2}{1} = {r=6}{},
  cell{8}{1} = {r=6}{},
  vline{2} = {2,8}{},
  hline{1-2,8,14} = {-}{},
  hline{3-7,9-13} = {2-3}{},
}
                & \textbf{Task Database}                                                                                                   & \textbf{Ground truth SQL query}                                                                                                                                   \\
\textbf{Easy}   & {List the name of teachers whose hometown \\is not “Little Lever Urban District. \\\textbf{(course\_teach)}}             & {SELECT name FROM teacher \\WHERE hometown != "little lever urban district”}                                                                                      \\
                & {What is the abbreviation \\for airline "JetBlue Airways" ? \\\textbf{(flight\_2)}}                                      & {SELECT Abbreviation FROM AIRLINES \\WHERE Airline = "JetBlue Airways”}                                                                                           \\
                & {List all the student details in \\reversed lexicographical order. \\\textbf{(student\_transcripts\_tracking)}}          & {SELECT other\_student\_details FROM Students \\ORDER BY other\_student\_details DESC}                                                                            \\
                & {What are the names of the \\singers who are not French citizens? \\\textbf{(singer)}}                                   & {SELECT Name FROM singer \\WHERE Citizenship != "France”}                                                                                                         \\
                & {How many ships ended up being 'Captured'?\\\textbf{(battle\_death)}}                                                    & {SELECT COUNT(*) FROM ship \\WHERE disposition\_of\_ship = 'Captured’}                                                                                            \\
                & {In which years cars were produced weighing \\no less than 3000 and no more than 4000?\\\textbf{(car\_1)}}               & {SELECT DISTINCT year FROM cars\_data \\WHERE weight BETWEEN 3000 AND 4000}                                                                                       \\
\textbf{Medium} & {Which airlines have less than 200 flights?\\\textbf{(flights\_2)}}                                                      & {SELECT T1.Airline FROM AIRLINES AS T1 \\JOIN FLIGHTS AS T2 ON T1.uid = T2.Airline \\GROUP BY T1.Airline HAVING COUNT(*)  200}                                    \\
                & {Who is the earliest graduate of the school? \\ List the first name, middle name, and last name.\\\textbf{(flights\_2)}} & {SELECT first\_name , middle\_name , last\_name \\FROM Students ORDER BY date\_left ASC LIMIT 1}                                                                  \\
                & {What are the countries having \\at least one car maker? \\ List name and id.\\\textbf{(car\_1)}}                        & {SELECT T1.CountryName , T1.CountryId \\FROM COUNTRIES \\AS T1 JOIN CAR\_MAKERS AS T2 \\ON T1.CountryId = T2.Country \\GROUP BY T1.CountryId HAVING COUNT(*) = 1} \\
                & {What is the official language used \\in the country the name of \\whose head of state is Beatrix?\\\textbf{(world\_1)}} & {SELECT T2.Language FROM country AS T1 \\JOIN countrylanguage AS T2 \\ON T1.Code = T2.CountryCode \\WHERE T1.HeadOfState = "Beatrix" \\AND T2.IsOfficial = "T”}   \\
                & {Find all airlines that have at least 10 flights.\\\textbf{(flights\_2)}}                                                & {SELECT T1.Airline FROM AIRLINES \\AS T1 JOIN FLIGHTS AS T2 ON T1.uid = T2.Airline \\GROUP BY T1.Airline HAVING COUNT(*)  10}                                     \\
                & {What are the codes of countries \\where Spanish is spoken by \\ the largest percentage of people?\\\textbf{(world\_1)}} & {SELECT CountryCode , MAX(Percentage) \\FROM countrylanguage \\WHERE language= SSpanish" GROUP BY CountryCode}                                                    
\end{tblr}
\end{table}

==> table/user_study_table.tex <==
\begin{table}
\centering
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
  & \textbf{Complete}
  & \textbf{Correct} 
  & $\rm \textbf{Acc.}$
  & \textbf{Skipped} \\ 
  \midrule

MISP        & 3.0   & 1.7    & 0.57   & 1.4   \\
DIY     & 5.4   &  3.5    &  0.68     & 0.8  \\
STEPS       & \textbf{6.7}   & \textbf{5.7}     & \textbf{0.86}  & \textbf{0.3}\\ 
\bottomrule
\end{tabular}%
}
\caption{User Performance (best results in bold). For all metrics, an ANOVA test indicated statistically significant mean differences across 3 tools ($p$-value < 0.01).}
\label{tab:task_completion}
\end{table}



